Linear Stochastic Thermodynamics

We study the thermodynamics of open systems weakly driven out-of-equilibrium by nonconservative and time-dependent forces using the linear regime of stochastic thermodynamics. We make use of conservation laws to identify the potential and nonconservative components of the forces. This allows us to formulate a unified near-equilibrium thermodynamics. For nonequilibrium steady states, we obtain an Onsager theory ensuring nonsingular response matrices that is consistent with phenomenological linear irreversible thermodynamics. For time-dependent driving protocols that do not produce nonconservative forces, we identify the equilibrium ensemble from which Green-Kubo relations are recovered. For arbitrary periodic drivings, the averaged entropy production (EP) is expressed as an independent sum over each driving frequency of non-negative contributions. These contributions are bilinear in the nonconservative and conservative forces and involve a novel generalized Onsager matrix that is symmetric. In the most general case of arbitrary time-dependent drivings, we advance a novel decomposition of the EP rate into two non-negative contributions - one solely due to nonconservative forces and the other solely due to deviation from the instantaneous steady-state - directly implying a minimum entropy production principle close to equilibrium. This setting reveals the geometric structure of near-equilibrium thermodynamics and generalizes previous approaches to cases with nonconservative forces.

==> texfiles/tolcolors.tex <==
\definecolor{tol-blue1}{rgb}{0.467,0.667,0.867}
\definecolor{tol-blue2}{RGB}{52, 101,164}
\definecolor{tol-blue3}{rgb}{0.067,0.267,0.467}

\definecolor{tol-green1}{rgb}{0.533,0.800,0.667}
\definecolor{tol-green2}{rgb}{0.267,0.667,0.467}
\definecolor{tol-green3}{rgb}{0.067,0.467,0.267}

\definecolor{tol-orange1}{rgb}{0.867,0.667,0.467}
\definecolor{tol-orange2}{RGB}{245,121,0}
\definecolor{tol-orange3}{rgb}{0.467,0.267,0.067}

\definecolor{tol-red1}{rgb}{0.867,0.467,0.533}
\definecolor{tol-red2}{rgb}{0.667,0.267,0.333}
\definecolor{tol-red3}{rgb}{0.467,0.067,0.133}

\definecolor{tol-yellow1}{rgb}{0.867,0.867,0.467}
\definecolor{tol-yellow2}{rgb}{0.667,0.667,0.267}
\definecolor{tol-yellow3}{rgb}{0.467,0.467,0.067}

